Typed compositional quantum computation with lenses

We propose a type-theoretic framework for describing and proving properties of quantum computations, in particular those presented as quantum circuits. Our proposal is based on an observation that, in the polymorphic type system of Coq, currying on quantum states allows us to apply quantum gates directly inside a complex circuit. By introducing a discrete notion of lens to control this currying, we are further able to separate the combinatorics of the circuit structure from the computational content of gates. We apply our development to define quantum circuits recursively from the bottom up, and prove their correctness compositionally.

==> mintedblock.tex <==
% https://tex.stackexchange.com/questions/376090/highlight-function-in-minted-with-background-color

\newif\ifFirstMintedPart
\makeatletter
\newenvironment{mintedBlock}{%
    \par
    \medskip%TODO
    \begingroup
        \setlength{\parskip}{0pt}%
        \setlength{\baselineskip}{0pt}%
        \setlength{\lineskip}{0pt}%
        \let\originalVspace=\vspace
        \renewcommand{\vspace}{\@ifnextchar*\@gobbletwo\@gobble}%
        \setlength{\fboxsep}{0pt}%
        \FirstMintedParttrue
        \originalVspace{2pt}%TODO
        \par
}{%
        % \par
        \originalVspace{-1em}%TODO
        \par
    \endgroup
    \medskip%TODO
}
\makeatother

\newminted{ssr}{frame=lines, tabsize=4}

\definecolor{llgray}{rgb}{0.95,0.95,0.95}

\newenvironment{goal}{%
    \VerbatimEnvironment
    \ifFirstMintedPart
        \newcommand\currentLine{firstnumber=1}%
    \else
        \newcommand\currentLine{firstnumber=last}%
    \fi
    \newcommand{\beginSsr}{\begin{ssrcode*}}%
    \expandafter\beginSsr\expandafter{%
        \currentLine,
        frame=none, 
        bgcolor=white,
        breaklines, % this is important!
        linenos,
    }%
}{%
    \end{ssrcode*}%
    \global\FirstMintedPartfalse
}

\newenvironment{tactic}{%
    \VerbatimEnvironment
    \ifFirstMintedPart
        \newcommand\currentLine{firstnumber=1}%
    \else
        \newcommand\currentLine{firstnumber=last}%
    \fi
    \newcommand{\beginSsr}{\begin{ssrcode*}}%
    \expandafter\beginSsr\expandafter{%
        \currentLine,
        frame=none,
        bgcolor=llgray,
        breaklines, % this is important!
        linenos,
        escapeinside=99,
    }%
}{%
    \end{ssrcode*}%
    \global\FirstMintedPartfalse
}

\newenvironment{sgoal}{%
    \VerbatimEnvironment
    \ifFirstMintedPart
        \newcommand\currentLine{firstnumber=1}%
    \else
        \newcommand\currentLine{firstnumber=last}%
    \fi
    \newcommand{\beginSsr}{\begin{ssrcode*}}%
    \expandafter\beginSsr\expandafter{%
        \currentLine,
        frame=none, 
        bgcolor=white,
        breaklines, % this is important!
        linenos,
        fontsize=\small,
    }%
}{%
    \end{ssrcode*}%
    \global\FirstMintedPartfalse
}

\newenvironment{stactic}{%
    \VerbatimEnvironment
    \ifFirstMintedPart
        \newcommand\currentLine{firstnumber=1}%
    \else
        \newcommand\currentLine{firstnumber=last}%
    \fi
    \newcommand{\beginSsr}{\begin{ssrcode*}}%
    \expandafter\beginSsr\expandafter{%
        \currentLine,
        frame=none,
        bgcolor=llgray,
        breaklines, % this is important!
        linenos,
        escapeinside=99,
        fontsize=\small,
    }%
}{%
    \end{ssrcode*}%
    \global\FirstMintedPartfalse
}

\newcommand{\colorMain}{green!10}%
\newcommand{\colorSum}{yellow!20}%

\iffalse
\begin{document}

\begin{mintedBlock}
    \begin{cpart}{}
        #include <stdio.h>
    \end{cpart}
    \begin{cpart}{}
    \end{cpart}
    \begin{cpart}{bgcolor=\colorSum}
        int sum(int summand1, int summand2)
        {
            return summand1 + summand2;
        }
    \end{cpart}
    \begin{cpart}{}
    \end{cpart}
    \begin{cpart}{bgcolor=\colorMain, escapeinside=~~}
        int main()
        {
            int summand1 = 1;
            int summand2 = 2;
            printf("%d + %d = %d\n", summand1, summand2, ~\linebreak~sum(summand1, summand2));
        }
    \end{cpart}
\end{mintedBlock}

\end{document}
\fi

